Building a Subspace of Policies for Scalable Continual Learning

The ability to continuously acquire new knowledge and skills is crucial for autonomous agents. Existing methods are typically based on either fixed-size models that struggle to learn a large number of diverse behaviors, or growing-size models that scale poorly with the number of tasks. In this work, we aim to strike a better balance between an agent's size and performance by designing a method that grows adaptively depending on the task sequence. We introduce Continual Subspace of Policies (CSP), a new approach that incrementally builds a subspace of policies for training a reinforcement learning agent on a sequence of tasks. The subspace's high expressivity allows CSP to perform well for many different tasks while growing sublinearly with the number of tasks. Our method does not suffer from forgetting and displays positive transfer to new tasks. CSP outperforms a number of popular baselines on a wide range of scenarios from two challenging domains, Brax (locomotion) and Continual World (manipulation).

==> algorithms/algorithm1.tex <==
\KwInputBis{$\bar\theta_{1}$,...,$\bar\theta_{K}$ (previous anchors), $n$ (budget), $\epsilon$ (threshold)}
\KwInput{$\phi$ (Critic), $\mathcal{R}$ (replay buffer)} 
Define $\bar\theta_{K+1} \leftarrow \frac{1}{K} \sum   \bar\theta_i$ (new anchor) \\
\For{$k=1,...,n$}{
    Sample $z \sim Dir \left ( K+1 \right )$ \\
    Set policy parameters $\theta_{z} \leftarrow \sum z_i  \bar\theta_i$ \\
    Collect and store $(s,a,r,s',d)$ in $\mathcal{R}$ by sampling $a \sim \pi_{\theta_{z}} \left (. |s \right )$\\
    \If{time to update}{Update $\bar\theta_{K+1}$ and $\phi$ using $\mathcal{R}$ and SAC algorithm}
}
Use $\mathcal{R}$ and $\phi$ to estimate: \\
    \begin{equation}
z^{*}_{K}\leftarrow \underset{z \in \Delta_K}{\arg\max}\:\:\phi(.,z)    
    \end{equation}
    \begin{equation}
z^{*}_{K+1}\leftarrow \underset{z \in \Delta_{K+1}}{\arg\max}\:\:\phi(.,z)
    \end{equation}
\eIf{$\phi(.,z^{*}_{K+1}) > (1 + \epsilon) \cdot \phi(.,z^{*}_{K})$}{\textbf{Return:\:}$\bar\theta_{1},...,\bar\theta_{K},\bar\theta_{K+1},\:\:z^{*}_{K+1}$}{\textbf{Return:\:}$\bar\theta_{1},...,\bar\theta_{K},\:\:z^*$}


==> tables/OLD_ant_4_tasks.tex <==
\begin{table*}[h!]
    \centering
    \caption{Detailed results of the short version (4 tasks) of our 4 Ant scenarios. Results presents mean and standard deviation of our 4 metrics, are split by scenario and method, and are averaged over 3 seeds.}
    \small
\begin{tabular}{llllll}
    \toprule
    & \textbf{Method} & \textbf{Performance} & \textbf{Transfer}  & \textbf{Forgetting} & \textbf{Growing Factor} \\ [0.5ex]
    \midrule
\parbox[t]{5mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{Forgetting scenario}}} 
&FT-1 &1.36 ± 0.29 &0.42 ± 0.26 &-0.06 ± 0.04 &\textbf{1.0} \\
&FT-L2 &1.73 ± 0.34 &0.61 ± 0.3 &0.12 ± 0.14 &2.0 \\
&EWC &1.83 ± 0.16 &0.81 ± 0.09 &0.02 ± 0.07 &3.0 \\
&PNN &0.77 ± 0.09 &-0.23 ± 0.09 &0.0 ± 0.0 &12.3 \\
&SAC-N &1.0 ± 0.32 &0.0 ± 0.32 &0.0 ± 0.0 &1.0 \\
&FT-N &\textbf{1.97 ± 0.11} &\textbf{0.97 ± 0.11} &0.0 ± 0.0 &4.0 \\
\cmidrule{2-6}
&CSP-MID &1.09 ± 0.11 &0.21 ± 0.16 &-0.11 ± 0.27 &3.38 ± 0.48 \\
&CSP-ORACLE &2.01 ± 0.07 &0.96 ± 0.04 &0.05 ± 0.03 &3.38 ± 0.48 \\
\cmidrule{2-6}
&CSP (ours) &1.78 ± 0.06 &0.78 ± 0.06 &\textbf{0.0 ± 0.0} &3.38 ± 0.48 \\
\midrule
\parbox[t]{5mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{Transfer scenario}}} 
&FT-1 &-0.12 ± 0.29 &-0.65 ± 0.7 &-0.47 ± 0.41 &\textbf{1.0} \\
&FT-L2 &0.85 ± 0.23 &-0.06 ± 0.29 &-0.09 ± 0.07 &2.0 \\
&EWC &0.53 ± 0.02 &-0.47 ± 0.02 &0.0 ± 0.0 &3.0 \\
&PNN &0.98 ± 0.02 &-0.02 ± 0.01 &0.0 ± 0.0 &12.3 \\
&SAC-N &1.0 ± 0.51 &0.0 ± 0.51 &0.0 ± 0.0 &1.0 \\
&FT-N &0.83 ± 0.47 &-0.17 ± 0.47 &0.0 ± 0.0 &4.0 \\
\cmidrule{2-6}
&CSP-MID &0.2 ± 0.04 &-0.23 ± 0.11 &-0.57 ± 0.08 &3.67 ± 0.47 \\
&CSP-ORACLE &1.51 ± 0.25 &0.49 ± 0.25 &0.02 ± 0.03 &3.67 ± 0.47 \\
\cmidrule{2-6}
&CSP (ours) &\textbf{1.41 ± 0.27} &\textbf{0.41 ± 0.27} &\textbf{0.0± 0.0} &3.67 ± 0.47 \\
\midrule
\parbox[t]{5mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{Distraction scenario}}} 
&FT-1 &0.26 ± 0.09 &-0.19 ± 0.16 &-0.56 ± 0.12 &\textbf{1.0} \\
&FT-L2 &0.46 ± 0.08 &-0.46 ± 0.03 &-0.08 ± 0.08 &2.0 \\
&EWC &0.42 ± 0.05 &-0.5 ± 0.03 &-0.07 ± 0.08 &3.0 \\
&PNN &0.72 ± 0.16 &-0.29 ± 0.16 &0.0 ± 0.0 &12.3 \\
&SAC-N &1.00 ± 0.05 &0.0 ± 0.05 &0.0 ± 0.0 &4.0 \\
&FT-N &0.89 ± 0.11 &-0.11 ± 0.11 &0.0 ± 0.0 &4.0 \\
\cmidrule{2-6}
&CSP-MID &0.21 ± 0.16 &-0.46 ± 0.07 &-0.32 ± 0.09 &3.0 ± 0.0 \\
&CSP-ORACLE &1.04 ± 0.04 &-0.01 ± 0.03 &0.05 ± 0.01 &3.0 ± 0.0 \\
\cmidrule{2-6}
&CSP (ours) &\textbf{0.94 ± 0.04} &\textbf{-0.06 ± 0.04} &\textbf{0.0± 0.0} &3.0 ± 0.0 \\
\midrule
\parbox[t]{5mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{Compositional scenario}}} 
&FT-1 &-0.84 ± 0.11 &-1.06 ± 0.25 &-0.78 ± 0.31 &\textbf{1.0} \\
&FT-L2 &0.12 ± 0.31 &-0.8 ± 0.17 &-0.08 ± 0.13 &2.0 \\
&EWC &0.26 ± 0.51 &0.06 ± 0.73 &-0.81 ± 1.0 &3.0 \\
&PNN &0.11 ± 0.35 &-0.89 ± 0.35 &0.0 ± 0.0 &12.3 \\
&SAC-N &1.00 ± 0.32 &0.0 ± 0.32 &0.0 ± 0.0 &4.0 \\
&FT-N &2.52 ± 0.03 &1.52 ± 0.03 &0.0 ± 0.0 &4.0 \\
\cmidrule{2-6}
&CSP-MID &2.29 ± 0.21 &1.28 ± 0.26 &0.0 ± 0.21 &3.33 ± 0.47 \\
&CSP-ORACLE &3.36 ± 0.71 &2.3 ± 0.65 &0.06 ± 0.06 &3.33 ± 0.47 \\
\cmidrule{2-6}
&CSP (ours) &\textbf{3.06 ± 0.77} &\textbf{2.06 ± 0.77} &\textbf{0.0 ± 0.0} &3.33 ± 0.47 \\
\midrule
\parbox[t]{5mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{\textbf{Aggregate}}}} 
&FT-1 &0.17 ± 0.2 &-0.37 ± 0.34 &-0.47 ± 0.22 &\textbf{1.0} \\
&FT-L2 &0.79 ± 0.24 &-0.18 ± 0.2 &-0.03 ± 0.11 &2.0 \\
&EWC &0.76 ± 0.19 &-0.03 ± 0.22 &-0.22 ± 0.29 &3.0 \\
&PNN &0.65 ± 0.16 &-0.36 ± 0.15 &0.0 ± 0.0 &12.3 \\
&SAC-N &1.0 ± 0.30 &0.00 ± 0.30 &0.0 ± 0.0 &2.5 \\
&FT-N &1.55 ± 0.18 &0.55 ± 0.18 &0.0 ± 0.0 &4.0 \\
\cmidrule{2-6}
&CSP-MID &0.95 ± 0.13 &0.2 ± 0.15 &-0.25 ± 0.16 &3.3 ± 0.4 \\
&CSP-ORACLE &1.98 ± 0.27 &0.94 ± 0.24 &0.05 ± 0.03 &3.3 ± 0.4 \\
\cmidrule{2-6}
&CSP (ours) &\textbf{1.8 ± 0.29} &\textbf{0.8 ± 0.29} &\textbf{0.0 ± 0.0} &3.3 ± 0.4 \\
\end{tabular}
\label{tab:ant_4_tasks}
\end{table*}

==> tables/OLD_ant_references.tex <==
\begin{table*}[h!]
    \centering
    \caption{Raw cumulative rewards obtained on each task of the 4 scenarios. These are obtained with a single policy learned from scratch (SAC-N) and the set of hyperparameters selected by the gridsearch of the FT-N method (see \ref{app:exp}). This explains why similar tasks have different averaged returns across scenarios. Results are averaged over 3 seeds.}
    \small
\begin{tabular}{l|l|l}
    & \textbf{Task} & \textbf{Cumulative rewards} \\ [0.5ex]
    \midrule
\multirow{4}{*}{Forgetting Scenario} &normal &3752 \\
&hugefeet &2841 \\
&rainfall &1596 \\
&moon &1401 \\
\midrule
\multirow{4}{*}{Transfer Scenario} & disableddiagonalfeet\_1 &3021 \\
& disableddiagonalfeet\_2 &4119 \\
& disabledforefeet &1014 \\
& disabledhindfeet &1021 \\
\midrule
\multirow{4}{*}{Distraction Scenario}
& normal &3542 \\
& inverted\_actions &4199 \\
& normal &3542 \\
& inverted\_actions &4199 \\
\midrule
\multirow{4}{*}{Compositional Scenario}
& disabled3feet\_1 &770 \\
& disabled3feet\_2 &641 \\
& disabledforefeet &201 \\
& disabledhindfeet &288 \\
\end{tabular}
\label{tab:ant_references}
\end{table*}

==> tables/OLD_halfcheetah_4_tasks.tex <==
\begin{table*}[h!]
    \centering
    \caption{Detailed results of the short version (4 tasks) of our 4 Halfcheetah scenarios. Results presents mean and standard deviation of our 4 metrics, are split by scenario and method, and are averaged over 3 seeds.}
    \small
\begin{tabular}{llllll}
    \toprule
    & \textbf{Method} & \textbf{Performance} & \textbf{Transfer}  & \textbf{Forgetting} & \textbf{Growing Factor} \\ [0.5ex]
    \midrule
\parbox[t]{5mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{Forgetting scenario}}} 
& FT-1 &0.99 ± 0.15 &0.57 ± 0.4 &-0.58 ± 0.27 &\textbf{1.0} \\
& FT-L2 &0.88 ± 0.26 &-0.13 ± 0.27 &0.0 ± 0.0 &2.0 \\
& EWC &1.05 ± 0.09 &0.08 ± 0.15 &-0.03 ± 0.06 &3.0 \\
& PNN &1.05 ± 0.45 &0.05 ± 0.45 &0.0 ± 0.0 &12.4 \\
& SAC-N &1.0 ± 0.35 &0.0 ± 0.35 &0.0 ± 0.0 &4.0 \\
& FT-N &\textbf{1.89 ± 0.2} &\textbf{0.89 ± 0.21} &0.0 ± 0.0 &4.0 \\
\cmidrule{2-6}
& CSP-MID &0.38 ± 0.4 &0.26 ± 0.37 &-0.88 ± 0.03 &3.0 ± 0.0 \\
& CSP-ORACLE &2.03 ± 0.01 &1.0 ± 0.02 &0.03 ± 0.03 &3.0 ± 0.0 \\
\cmidrule{2-6}
& CSP (ours) &1.76 ± 0.08 &0.76 ± 0.08 &\textbf{0.0 ± 0.0} &3.0 ± 0.0 \\
\midrule
\parbox[t]{5mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{Transfer scenario}}} & FT-1 &0.45 ± 0.03 &-0.07 ± 0.08 &-0.47 ± 0.05 &\textbf{1.0} \\
&FT-L2 &0.35 ± 0.09 &-0.49 ± 0.18 &-0.16 ± 0.09 &2.0 \\
&EWC &0.21 ± 0.01 &-0.79 ± 0.0 &0.0 ± 0.0 &3.0 \\
&PNN &0.84 ± 0.13 &-0.17 ± 0.13 &0.0 ± 0.0 &12.4 \\
&SAC-N &1.0 ± 0.02 &0.0 ± 0.02 &0.0 ± 0.0 &4.0 \\
&FT-N &0.94 ± 0.05 &-0.06 ± 0.05 &0.0 ± 0.0 &4.0 \\
\cmidrule{2-6}
&CSP-MID &0.52 ± 0.08 &-0.19 ± 0.07 &-0.29 ± 0.11 &3.33 ± 0.47 \\
&CSP-ORACLE &1.14 ± 0.07 &0.14 ± 0.04 &0.0 ± 0.03 &3.33 ± 0.47 \\
\cmidrule{2-6}
&CSP (ours) &\textbf{0.98 ± 0.06} &\textbf{-0.03 ± 0.06} &\textbf{0.0 ± 0.0} &3.33 ± 0.47 \\
\midrule
\parbox[t]{5mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{Distraction scenario}}} &FT-1 &0.36 ± 0.06 &-0.18 ± 0.06 &-0.45 ± 0.12 &\textbf{1.0} \\
&FT-L2 &0.53 ± 0.05 &-0.47 ± 0.05 &0.0 ± 0.0 &2.0 \\
&EWC &0.78 ± 0.41 &-0.2 ± 0.39 &-0.02 ± 0.08 &3.0 \\
&PNN &1.09 ± 0.03 &0.1 ± 0.03 &0.0 ± 0.0 &12.4 \\
&SAC-N &1.0 ± 0.18 &0.0 ± 0.18 &0.0 ± 0.0 &4.0 \\
&FT-N &1.11 ± 0.03 &0.11 ± 0.03 &0.0 ± 0.0 &4.0 \\
\cmidrule{2-6}
&CSP-MID &0.43 ± 0.12 &-0.07 ± 0.1 &-0.5 ± 0.18 &3.0 ± 0.82 \\
&CSP-ORACLE &1.29 ± 0.08 &0.28 ± 0.07 &0.01 ± 0.0 &3.0 ± 0.82 \\
\cmidrule{2-6}
&CSP (ours) &\textbf{1.13 ± 0.09} &\textbf{0.13 ± 0.09} &\textbf{0.0 ± 0.0} &3.0 ± 0.82 \\
\midrule
\parbox[t]{5mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{Compositional scenario}}} &FT-1 &1.19 ± 0.09 &0.33 ± 0.04 &-0.15 ± 0.05 &\textbf{1.0} \\
&FT-L2 &1.2 ± 0.13 &0.28 ± 0.08 &-0.08 ± 0.05 &2.0 \\
&EWC &1.0 ± 0.17 &0.07 ± 0.16 &-0.07 ± 0.03 &3.0 \\
&PNN &1.0 ± 0.28 &0.0 ± 0.29 &0.0 ± 0.0 &12.4 \\
&SAC-N &1.0 ± 0.2 &0.0 ± 0.2 &0.0 ± 0.0 &4.0 \\
&FT-N &\textbf{1.5 ± 0.18} &\textbf{0.5 ± 0.17} &0.0 ± 0.0 &4.0 \\
\cmidrule{2-6}
&CSP-MID &.72 ± 0.12 &-0.04 ± 0.22 &-0.24 ± 0.11 &3.33 ± 0.47 \\
&CSP-ORACLE &1.58 ± 0.05 &0.59 ± 0.05 &-0.01 ± 0.0 &3.33 ± 0.47 \\
\cmidrule{2-6}
&CSP (ours) &1.39 ± 0.1 &0.39 ± 0.1 &\textbf{0.0 ± 0.0} &3.33 ± 0.47 \\
\midrule
\parbox[t]{5mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{\textbf{Aggregate}}}} &FT-1 &0.75 ± 0.08 &0.16 ± 0.15 &-0.41 ± 0.12 &\textbf{1.0} \\
&FT-L2 &0.74 ± 0.13 &-0.2 ± 0.15 &-0.06 ± 0.04 &2.0 \\
&EWC &0.76 ± 0.17 &-0.21 ± 0.18 &-0.03 ± 0.04 &3.0 \\
&PNN &1 ± 0.22 &-0.01 ± 0.23 &0 ± 0 &12.4 \\
&SAC-N &1 ± 0.19 &0 ± 0.19 &0 ± 0 &4.0 \\
&FT-N &\textbf{1.36 ± 0.12} &\textbf{0.36 ± 0.12} &0 ± 0 &4.0 \\
\cmidrule{2-6}
&CSP-MID &0.51 ± 0.18 &-0.01 ± 0.19 &-0.48 ± 0.11 &3.2 ± 0.4 \\
&CSP-ORACLE &1.51 ± 0.05 &0.5 ± 0.05 &0.01 ± 0.02 &3.2 ± 0.4 \\
\cmidrule{2-6}
&CSP (ours) &1.32 ± 0.08 &0.31 ± 0.08 &\textbf{0 ± 0.0} &3.2 ± 0.4 \\
\end{tabular}
\label{tab:halfcheetah_4_tasks}
\end{table*}

==> tables/OLD_halfcheetah_8_tasks.tex <==
\begin{table*}[h!]
    \centering
    \caption{Detailed results of the long version (8 tasks) of our 4 Halfcheetah scenarios. Results presents mean and standard deviation of our 4 metrics, are split by scenario and method, and are averaged over 10 seeds.}
    \small
\begin{tabular}{llllll}
    \toprule
    & \textbf{Method} & \textbf{Performance} & \textbf{Transfer}  & \textbf{Forgetting} & \textbf{Growing Factor} \\ [0.5ex]
    \midrule
\parbox[t]{5mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{Forgetting scenario}}} 
&FT-1 &0.95 ± 0.37 &0.79 ± 0.34 &-0.84 ± 0.08 &\textbf{1.0} \\
&FT-L2 &1.07 ± 0.12 &0.53 ± 0.25 &-0.46 ± 0.15 &2.0 \\
&EWC &1.37 ± 0.33 &0.77 ± 0.21 &-0.4 ± 0.12 &3.0 \\
&PNN &1.35 ± 0.45 &0.35 ± 0.45 &0.0 ± 0.0 &47.3 \\
&FT-N &1.68 ± 0.15 &0.68 ± 0.15 &0.0 ± 0.0 &8.0 \\
\cmidrule{2-6}
&CSP-MID &0.55 ± 0.4 &-0.1 ± 0.45 &-0.36 ± 0.15 &4.33 ± 1.7 \\
&CSP-ORACLE &1.98 ± 0.04 &0.87 ± 0.13 &0.11 ± 0.14 &4.33 ± 1.7 \\
\cmidrule{2-6}
&CSP (ours) &\textbf{1.69 ± 0.12} &\textbf{0.69 ± 0.12} &\textbf{0. ± 0.0} &4.33 ± 1.7 \\
\midrule
\parbox[t]{5mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{Transfer scenario}}} &FT-1 &0.42 ± 0.07 &-0.16 ± 0.07 &-0.42 ± 0.07 &\textbf{1.0} \\
&FT-L2 &0.37 ± 0.07 &-0.22 ± 0.04 &-0.42 ± 0.09 &2.0 \\
&EWC &0.52 ± 0.08 &-0.36 ± 0.05 &-0.11 ± 0.05 &3.0 \\
&PNN &0.87 ± 0.08 &-0.13 ± 0.08 &0.0 ± 0.0 &47.3 \\
&FT-N &0.89 ± 0.12 &-0.11 ± 0.12 &0.0 ± 0.0 &8.0 \\
\cmidrule{2-6}
&CSP-MID &0.62 ± 0.17 &-0.29 ± 0.13 &-0.09 ± 0.11 &4.67 ± 0.47 \\
&CSP-ORACLE &1.2 ± 0.06 &0.15 ± 0.09 &0.05 ± 0.03 &4.67 ± 0.47 \\
\cmidrule{2-6}
&CSP (ours) &\textbf{0.97 ± 0.08} &\textbf{-0.04 ± 0.08} &\textbf{0.0 ± 0.0} &4.67 ± 0.47 \\
\midrule
\parbox[t]{5mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{Distraction scenario}}} &FT-1 &0.36 ± 0.18 &-0.24 ± 0.13 &-0.39 ± 0.09 &\textbf{1.0} \\
&FT-L2 &0.61 ± 0.08 &-0.38 ± 0.06 &-0.02 ± 0.02 &2.0 \\
&EWC &0.66 ± 0.05 &-0.3 ± 0.03 &-0.04 ± 0.04 &3.0 \\
&PNN &0.97 ± 0.09 &-0.03 ± 0.09 &0.0 ± 0.0 &47.3 \\
&FT-N &0.84 ± 0.03 &-0.16 ± 0.03 &0.0 ± 0.0 &8.0 \\
\cmidrule{2-6}
&CSP-MID &0.54 ± 0.03 &-0.31 ± 0.04 &-0.14 ± 0.04 &2.0 ± 0.0 \\
&CSP-ORACLE &1.27 ± 0.03 &0.26 ± 0.04 &0.01 ± 0.0 &2.0 ± 0.0 \\
\cmidrule{2-6}
&CSP (ours) &\textbf{1.18 ± 0.03} &\textbf{0.18 ± 0.03} &\textbf{0.0 ± 0.0} &2.0 ± 0.0 \\
\midrule
\parbox[t]{5mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{Compositional scenario}}} &FT-1 &1.28 ± 0.03 &0.42 ± 0.02 &-0.13 ± 0.04 &1.0 \\
&FT-L2 &1.19 ± 0.09 &0.41 ± 0.21 &-0.22 ± 0.13 &2.0 \\
&EWC &1.38 ± 0.11 &0.43 ± 0.15 &-0.05 ± 0.13 &3.0 \\
&PNN &1.04 ± 0.07 &0.04 ± 0.08 &0.0 ± 0.0 &47.3 \\
&FT-N &\textbf{1.48 ± 0.08} &\textbf{0.48 ± 0.08} &0.0 ± 0.0 &8.0 \\
\cmidrule{2-6}
&CSP-MID &0.84 ± 0.09 &-0.16 ± 0.06 &0.0 ± 0.04 &5.0 ± 0.82 \\
&CSP-ORACLE &1.68 ± 0.22 &0.64 ± 0.12 &0.04 ± 0.1 &5.0 ± 0.82 \\
\cmidrule{2-6}
&CSP (ours) &1.42 ± 0.03 &0.42 ± 0.03 &\textbf{0.0 ± 0.0} &5.0 ± 0.82 \\
\midrule
\parbox[t]{5mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{Aggregate}}}} &FT-1 &0.75 ± 0.16 &0.2 ± 0.14 &-0.45 ± 0.07 &1.0 \\
&FT-L2 &0.81 ± 0.09 &0.09 ± 0.14 &-0.28 ± 0.1 &2.0 \\
&EWC &1.22 ± 0.1 &0.22 ± 0.1 &0 ± 0 &8.0 \\
&PNN &0.98 ± 0.14 &0.14 ± 0.11 &-0.15 ± 0.09 &3.0 \\
&FT-N &1.06 ± 0.17 &0.06 ± 0.18 &0 ± 0 &47.3 \\
\cmidrule{2-6}
&CSP-MID &0.64 ± 0.17 &-0.22 ± 0.17 &-0.15 ± 0.09 &4 ± 0.7 \\
&CSP-ORACLE &1.53 ± 0.09 &0.48 ± 0.1 &0.05 ± 0.07 &4 ± 0.7 \\
\cmidrule{2-6}
&CSP (ours) &\textbf{1.32 ± 0.07} &\textbf{0.31 ± 0.07} &\textbf{0 ± 0.0} &4 ± 0.7 \\
\end{tabular}
\label{tab:halfcheetah_8_tasks}
\end{table*}

==> tables/OLD_halfcheetah_references.tex <==
\begin{table*}[h!]
    \centering
    \caption{Raw cumulative rewards obtained on each task of the 4 scenarios. These are obtained with a single policy learned from scratch (SAC-N) and the set of hyperparameters selected by the gridsearch of the FT-N method (see \ref{app:exp}). This explains why similar tasks have different averaged returns across scenarios. Results are averaged over 3 seeds.}
    \small
\begin{tabular}{c|l|l|l}
    & \textbf{Scenario} & \textbf{Task} & \textbf{Cumulative rewards} \\ [0.5ex]
    \midrule
\parbox[t]{5mm}{\multirow{16}{*}{\rotatebox[origin=c]{90}{Halfcheetah}}} 
& \multirow{4}{*}{Forgetting Scenario} & hugefoot &2209 \\
&  & moon &2982 \\
&  & carrystuff &6309 \\
&  & rainfall &1001 \\
\cmidrule{2-4}
&  \multirow{4}{*}{Transfer Scenario} & carrystuff\_hugegravity &7233 \\
&  &moon &3599 \\
&  &defectivemodule &5909 \\
& &hugefoot\_rainfall &2942 \\
\cmidrule{2-4}
& \multirow{4}{*}{Distraction Scenario}&normal &4932 \\
& &inverted\_actions &5833 \\
& &normal &4932 \\
& &inverted\_actions &5833 \\
\cmidrule{2-4}
& \multirow{4}{*}{Compositional Scenario}&tinyfoot &6311 \\
& &moon &3932 \\
& &carrystuff\_hugegravity &6319 \\
& &tinyfoot\_moon &1355 \\
\toprule
\parbox[t]{5mm}{\multirow{16}{*}{\rotatebox[origin=c]{90}{Ant}}} 
& \multirow{4}{*}{Forgetting Scenario} &normal &3752 \\
& &hugefeet &2841 \\
& &rainfall &1596 \\
& &moon &1401 \\
\cmidrule{2-4}
& \multirow{4}{*}{Transfer Scenario} & disableddiagonalfeet\_1 & 3021 \\
& & disableddiagonalfeet\_2 &4119 \\
& & disabledforefeet &1014 \\
& & disabledhindfeet &1021 \\
\cmidrule{2-4}
& \multirow{4}{*}{Distraction Scenario} & normal &3542 \\
& & inverted\_actions &4199 \\
& & normal &3542 \\
& & inverted\_actions &4199 \\
\cmidrule{2-4}
& \multirow{4}{*}{Compositional Scenario} & disabled3feet\_1 &770 \\
& & disabled3feet\_2 &641 \\
& & disabledforefeet &201 \\
& & disabledhindfeet &288 \\
\toprule
\parbox[t]{5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Humanoid}}} 
& & normal & 1958 \\
& & moon & 1691 \\
& & carrystuff & 2379 \\
& & tinyfeet & 1711 \\
\end{tabular}
\label{tab:halfcheetah_references}
\end{table*}

==> tables/OLD_humanoid_references.tex <==
\begin{table*}[h!]
    \centering
    \caption{Raw cumulative rewards obtained on each task of the humanoid scenario. These are obtained with a single policy learned from scratch (SAC-N) and the set of hyperparameters selected by the gridsearch of the FT-N method (see \ref{app:exp}). Results are averaged over 5 seeds.}
    \small
\begin{tabular}{l|l}
    \textbf{Task} & \textbf{Cumulative rewards} \\ [0.5ex]
    \midrule
normal & 1958 \\
moon & 1691 \\
carrystuff & 2379 \\
tinyfeet & 1711 \\
\end{tabular}
\label{tab:humanoid_references}
\end{table*}
			

==> tables/ant_hps.tex <==
\begin{table}[h!]
\begin{center}
\caption{Hyper-parameters selected for each Ant scenario. They have been selected on short versions. For the long versions, we ran the same set of selected hyperparameters.}
\label{tab:ant_hps}
\begin{tabular}{l|c|c|c|c} \toprule
    \textbf{Hyper-parameter} & \multicolumn{4}{c}{\textbf{Scenario}} \\
    & Forgetting & Transfer & Distraction & Compositional \\\hline
    lr policy &  $0.001$ & $0.001$ & $0.001$ & $0.0003$ \\
    lr critic &  $0.001$ & $0.001$ & $0.001$ & $0.0003$ \\
    reward scaling &  $10.$ & $1.$ & $1.$ & $10.$ \\
    target output std &  $0.05$ & $0.05$ & $0.1$ & $0.1$ \\
    policy update delay &  $2$ & $2$ & $2$ & $4$ \\
    target update delay  &  $4$ & $2$ & $4$ & $4$ \\
\\\toprule
\multicolumn{5}{c}{FT-L2} \\ 
    \hline
    regularization coefficient &  $10^4$ & $10^0$ & $10^0$ & $10^2$ \\ \\\toprule
\multicolumn{5}{c}{EWC} \\ 
    \hline
    regularization coefficient &  $10^{-2}$ & $10^{4}$ & $10^{2}$ & $10^{-2}$ \\ \\\toprule
    \multicolumn{5}{c}{CSP} \\ 
    \hline
    threshold &  $0.1$ & $0.1$ & $0.1$ & $0.1$ \\
    combination rollout length &  $100$ & $100$ & $100$ & $20$ \\
    distribution type &  peaked & peaked & peaked & peaked \\
\end{tabular}
\end{center}
\end{table}

==> tables/halfcheetah_hps.tex <==
\begin{table}[h!]
\begin{center}
\caption{Hyper-parameters selected for each HalfCheetah scenario. They have been selected on short versions. For the long versions, we ran the same set of selected hyperparameters.}
\label{tab:halfcheetah_hps}
\begin{tabular}{l|c|c|c|c} \toprule
    \textbf{Hyper-parameter} & \multicolumn{4}{c}{\textbf{Scenario}} \\
    & Forgetting & Transfer & Distraction & Compositional \\\hline
    lr policy &  $0.001$ & $0.0003$ & $0.001$ & $0.0003$ \\
    lr critic &  $0.0003$ & $0.0003$ & $0.001$ & $0.0003$ \\
    reward scaling &  $1.$ & $1.$ & $1.$ & $10.$ \\
    target output std &  $0.1$ & $0.05$ & $0.1$ & $0.1$ \\
    policy update delay &  $2$ & $2$ & $4$ & $4$ \\
    target update delay  &  $2$ & $2$ & $2$ & $4$ \\
\\\toprule
\multicolumn{5}{c}{FT-L2} \\ 
    \hline
    regularization coefficient &  $10^4$ & $10^0$ & $10^2$ & $10^2$ \\ \\\toprule
\multicolumn{5}{c}{EWC} \\ 
    \hline
    regularization coefficient &  $10^{-2}$ & $10^{0}$ & $10^{-2}$ & $10^{0}$ \\ \\\toprule
    \multicolumn{5}{c}{CSP} \\ 
    \hline
    threshold &  $0.1$ & $0.1$ & $0.1$ & $0.1$ \\
    combination rollout length &  $100$ & $20$ & $20$ & $100$ \\
    distribution type &  peaked & peaked & flat & flat \\
\end{tabular}
\end{center}
\end{table}

==> tables/humanoid_hps.tex <==
\begin{table}[H]
\begin{center}
\caption{Hyper-parameters selected for the Humanoid scenario.}
\label{tab:humanoid_hps}
\begin{tabular}{l|c} \toprule
    \textbf{Hyper-parameter} & \textbf{Scenario} \\
    \hline
    lr policy &  $0.001$ \\
    lr critic &  $0.0003$  \\
    reward scaling &  $0.1$ \\
    target output std &  $0.1$\\
    policy update delay &  $1$ \\
    target update delay  &  $1$ \\
\\\toprule
\multicolumn{2}{c}{FT-L2} \\ 
    \hline
    regularization coefficient &  $10^{-2}$ \\ \\\toprule
\multicolumn{2}{c}{EWC} \\ 
    \hline
    regularization coefficient &  $10^{-2}$  \\ \\\toprule
    \multicolumn{2}{c}{CSP} \\ 
    \hline
    threshold &  $0.1$ \\
    combination rollout length &  $100$ \\
    distribution type &  peaked \\
\end{tabular}
\end{center}
\end{table}
